SMIR: Efficient Synthetic Data Pipeline To Improve Multi-Image Reasoning

Vision-Language Models (VLMs) excel at understanding single images, aided by high-quality instruction datasets. However, multi-image reasoning remains underexplored in the open-source community due to two key challenges: (1) scaling datasets with correlated images and complex reasoning instructions is resource-intensive, and (2) robust evaluation benchmarks for multi-image tasks are lacking. To address this, we introduce SMiR, a synthetic data-generation pipeline for multi-image reasoning, along with a high-quality dataset generated using this pipeline. SMiR efficiently extracts correlated images via multimodal embeddings, integrates visual and descriptive information, and leverages open-source LLMs to generate quality instructions. Using this approach, we produce 160K synthetic training samples, offering a cost-effective alternative to closed-source solutions. Additionally, we present SMiR-Bench, a multi-image reasoning benchmark comprising 200 diverse examples across seven complex reasoning tasks. SMiR-Bench is multi-turn and employs a VLM judge to evaluate free-form responses, providing a comprehensive assessment of model expressiveness and reasoning capability across modalities. We demonstrate the effectiveness of SMiR by fine-tuning open-source VLMs and evaluating them on SMiR-Bench.

==> scratch.tex <==
% Consider a question like: \textbf{Compare the behaviors and characteristics shown in these images. How do they demonstrate different aspects of survival and adaptation?} Previous methods may match it with a relevant image of a dog alongside completely unrelated images like a drone hovering in the air and shipping containers at a port. While the question naturally applies to analyzing an animal's behavioral adaptations, its pairing with technological and industrial objects (drones, logistics, etc.) forces superficial comparisons that dilute the biological focus of the inquiry. This makes the task easier, as the unrelated items can only be discussed through loose metaphorical connections to survival and adaptation. The example is shown in Figure \ref{fig:comparison}.


In contrast, comparing related images—like a series of different animals in their natural habitats—demands a deeper understanding of predator behavior and ecological adaptation. Here, the task requires a more nuanced comparison of hunting techniques, territorial behaviors, and social structures within the same family of species. 

% While we do not have full visibility into how open-source models are trained, a reasonable assumption for their underperformance in multi-image reasoning tasks is the advantage closed-source models have in terms of training datasets. Closed-source developers likely benefit from access to large, high-quality datasets, which are critical for training advanced models capable of reasoning across multiple images. In contrast, open-source models may face limitations in accessing or constructing datasets that are specifically tailored to these tasks, which impacts their overall performance.

One major challenge lies in collecting and curating large-scale datasets with highly correlated images. Identifying meaningful connections between images requires vast amounts of data and sophisticated algorithms, which most multi-image instruction-tuning datasets lack. For example, MANTIS \citep{jiang2024mantis} often pairs unrelated images in the same reasoning task, unintentionally simplifying the challenge. An example of such a case is shown in \cref{fig:comparison}. MMDU-45K \citep{liu2024mmdu} attempts to address this by clustering image captions and category tags, but it overlooks the crucial visual relationships that may not be available only via caption. These shortcomings highlight the need for datasets with truly correlated images to foster complex multi-image reasoning tasks that better reflect real-world analytical challenges.

Second, scaling up the number of highly correlated images presents significant challenges. Existing datasets such as MANTIS, MMDU-45K, and MultiInstruct \citep{xu2022multiinstruct} require extensive human curation and annotation, resulting in a labor-intensive and time-consuming process. To minimize human effort, researchers have leveraged GPT-4 family models \citep{peng2023instruction, wang2023see} to generate synthetic datasets—including MMInstruct \citep{liu2024mminstruct}, Multimodal ArXiv \citep{li2024multimodal}, MIMIC-IT \citep{li2023mimic}, StableLLaVA-Instruct \citep{li2023stablellava}, and SVIT-Instruct \citep{zhao2023svit}. However, this method proves expensive and difficult to scale effectively. 

Third, evaluating multi-image reasoning is challenging due to the limitations of traditional assessment methods. Multiple-choice formats, used in previous multi-image reasoning benchmarks such as MMIU \citep{meng2024mmiu}, BLINK \citep{fu2024blink}, MuirBench \citep{wang2024muirbench}, MMMU \citep{yue2024mmmu}, fail to capture the nuanced reasoning process and justifications behind a model's answers. This is problematic because models can achieve similar performance on multiple-choice tasks while having vastly different reasoning capabilities. In contrast, free-form responses allow models to demonstrate their thought processes, providing a more comprehensive evaluation of their true reasoning abilities and distinguishing between models that rely on superficial pattern matching and those with a deeper understanding. In addition, benchmarks with short-answer components such as MIBench \citep{liu2024mibench} are not multi-turn, unable to replicate a real-world conversation that includes multi-images.

To address these challenges, we propose a synthetic data generation pipeline, \textsc{SMiR}, for multi-image reasoning, along with a human-annotated evaluation benchmark, \textsc{SMiR-Bench}. \textsc{SMiR} generates correlated and challenging multi-image reasoning questions, while \textsc{SMiR-Bench} evaluates models using free-response tasks in complex multi-image scenarios.

Our contributions are as follows:

\begin{itemize}

\item We present \textsc{SMiR}, a pipeline for multi-image instruction tuning. To construct \textsc{SMiR}, we apply existing algorithms in a novel way to collect multiple images with high correlation. Our approach combines cluster sampling for data quality robustness and graph iteration sampling for diversity. Both algorithms leverage multimodal embeddings that integrate image and caption information to effectively group correlated images, enabling challenging multi-image instruction tuning scenarios.

\item We develop a scalable synthetic multimodal data generation pipeline that leverages open-source LLMs such as Meta Llama 3.1 70B Instruct Turbo \citep{dubey2024llama}. This approach eliminates the need for expensive closed-source models, reducing costs by up to 50 times and increasing speed by up to 10 times \citep{kirkovska2024llama}, while significantly minimizing human annotation efforts.

\item We present a new multimodal evaluation benchmark that uses multi-turn interactions and free-form responses to assess both final answers and reasoning processes in complex multi-image tasks. The evaluation is conducted pairwise, directly comparing model performances. Using reference answers from GPT-4-Turbo and other open-source models as baselines, we observe up to an 8\% improvement in win rate for instruction-tuned models trained on the \textsc{SMiR} dataset.

\end{itemize}
